On the Generative Capacity of Contextual Grammars with Strictly Locally Testable Selection Languages

We continue the research on the generative capacity of contextual grammars where contexts are adjoined around whole words (externally) or around subwords (internally) which belong to special regular selection languages. All languages generated by contextual grammars where all selection languages are elements of a certain subregular language family form again a language family. We investigate contextual grammars with strictly locally testable selection languages and compare those families to families which are based on finite, monoidal, nilpotent, combinational, definite, suffix-closed, ordered, commutative, circular, non-counting, power-separating, or union-free languages.

==> eptcsdata.tex <==
\providecommand{\firstpage}{65}
\providecommand{\publicationstatus}{H. Bordihn, G. Horv\'ath, G. Vaszil (Eds.): 12th International Workshop on\\Non-Classical Models of Automata and Applications (NCMA 2022)\\
EPTCS 367, 2022, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.367.5}{10.4204/EPTCS.367.5}}

